Evaluation of Automatic Video Captioning Using Direct Assessment

We present Direct Assessment, a method for manually assessing the quality of automatically-generated captions for video. Evaluating the accuracy of video captions is particularly difficult because for any given video clip there is no definitive ground truth or correct answer against which to measure. Automatic metrics for comparing automatic video captions against a manual caption such as BLEU and METEOR, drawn from techniques used in evaluating machine translation, were used in the TRECVid video captioning task in 2016 but these are shown to have weaknesses. The work presented here brings human assessment into the evaluation by crowdsourcing how well a caption describes a video. We automatically degrade the quality of some sample captions which are assessed manually and from this we are able to rate the quality of the human assessors, a factor we take into account in the evaluation. Using data from the TRECVid video-to-text task in 2016, we show how our direct assessment method is replicable and robust and should scale to where there many caption-generation techniques to be evaluated.

==> vtt.tex <==
Automatic annotation of videos using natural language text descriptions has been a long-standing goal of computer vision. The task involves understanding of many concepts such as objects, actions, scenes, person-object relations, the temporal order of events throughout the video and many others. In recent years there have been major advances in computer vision techniques which enabled researchers to start practical work on solving the challenges posed in video captioning. 

There are many use case application scenarios which can greatly benefit from  technology such as video summarization in the form of natural language, including facilitating the search and browsing of video archives using such descriptions, describing videos to the blind, etc. In addition, learning video interpretation and temporal relations among events in a video will likely contribute to other computer vision tasks, such as prediction of future events from the video. 

This year a new showcase/pilot task was proposed and launched within TRECVid which we refer to as ``Video to Text Description'' (VTT) and describe in this section.  

\subsection{Data}
A dataset of more than 30k Twitter Vine videos has been collected automatically. Each video has a total duration of about 6 s. In this showcase/pilot task a subset of 2\,000 Vine videos was randomly selected and annotated manually twice by two different annotators. In total, 4 non-overlapping sets of 500 videos each were given to 8 annotators to generate a total of 4\,000 text descriptions. Those 4\,000 text descriptions were split into 2 sets corresponding to the original 2\,000 videos. Annotators were asked to include and combine into 1 sentence, if appropriate and available, four facets of the video they are describing:

\begin{itemize}
\item{Who is the video describing (e.g. concrete objects and beings, kinds of persons, animals, or things)}
\item{What are the objects and beings doing? (generic actions, conditions/state or events)}
\item{Where is the video taken (e.g. locale, site, place, geographic location, architectural)}
\item{When is the video taken (e.g. time of day, season)}
\end{itemize}


\subsection{System task}
The task set for participants was as follows: given a set of about 2\,000 URLs of Vine videos and two sets (A and B) of text descriptions (each composed of 2\,000 sentences), systems were asked to work and submit results for at least one of two subtasks:

\begin{itemize}
\item{Matching and Ranking: Return for each video URL a ranked list of the most likely text description that corresponds (was annotated) to the video from each of the sets A and B.}

\item{Description Generation: Automatically generate for each video URL a text description (1 sentence) independently and without taking into consideration the existence of sets A and B.} 
\end{itemize}


\subsection{Evaluation}
The matching and ranking subtask scoring was done automatically against the ground truth using mean inverted rank at which the annotated item is found. The Description generation subtask scoring was done automatically using  standard metrics from machine translation (MT) including METEOR \cite{banerjee2005meteor} and BLEU \cite{papineni2002bleu}. BLEU (bilingual evaluation understudy) is a metric used in MT and was one of the first metrics to achieve a high correlation with human judgements of quality. It is known to perform more poorly if it is used to evaluate the quality of individual sentence variations rather than sentence variations at a corpus level. In the VTT task the videos are independent thus there is no corpus to work from, so our expectations are lowered when it comes to evaluation by BLEU.  METEOR (Metric for Evaluation of Translation with explicit ORdering) is based on the harmonic mean of unigram or n-gram precision and recall, in terms of overlap between two input sentences. It redresses some of the shortfalls of BLEU such as better matching synonyms and stemming, though the two measures seem to be used together in evaluating MT.   

Systems taking part in VTT were encouraged to take into consideration and use the four facets that annotators used as a guideline to generate their automated descriptions. In addition to using MT metrics, an experimental semantic similarity metric (STS) \cite{han2013umbc} was applied. This metric measures how semantically similar the submitted description is to the ground truth descriptions (both A and B).
In total, 11 teams signed up for the pilot/showcase task and 7 of those finished, submitting 46 individual runs to the matching and ranking subtask and 16 runs to the description generation subtask. 

\subsection{Results}

Readers should see the online proceedings for individual teams' performance and runs but here we present a high-level overview.

The first set of results for the caption-ranking sub-task are shown in Figures \ref{vtt.match.rank.tv16} and \ref{vtt.match.rank.tv16.a.b} and shows the mean inverted rank scores for all submitted runs, color-coded by participating group. From Figure~\ref{vtt.match.rank.tv16} we can see that submitted runs from different groups cluster together indicating each group submitted runs which were slight variants of each other. To interpret these results we can say that with a mean inverted rank value of greater than 0.1, on average systems can find the correct caption from a set of 2\,000 captions, at rank position 9 or 10.

Figure~\ref{vtt.match.rank.tv16.a.b} shows the same results but differentiating the A runs from B runs and from this we can see that systems seem to perform better on the B runs than on the A runs, though what that means is not very clear.

If we explore these results a bit deeper, then Figure~\ref{vtt.top3.setA} shows the rank positions at which the top 3 videos from 2\,000, in terms of how ``easy'' they were to rank, were ranked by the submitting groups.

Video number 324, for example, was found within the top-1p rank positions by 5 of the runs, while for some of the runs it was not located until almost rank position 1\,000. This demonstrates the variable difficulty in this task, some systems perform well on some videos but badly on others.

The videos shown in Figure \ref{vtt.samples.easy}, for example, are among the easiest to rank highly, right across the submitted runs with their captions being {\em ``a woman and a man are kissing each other''} and {\em ``a dog imitating a baby crawling across the floor in a living room''}. On the other hand, the videos in Figure~\ref{vtt.samples.hard} are among the most challenging with their captions being {\em ``3 balls hover in front of a man''} and {\em ``a person wearing a costume and carrying a chainsaw''}. What makes these latter two videos most challenging is the unusual nature of the actions that take place. In the first case the 3 basketballs do hover in front of the subject as it is a video of a magic trick, and in the second case there is a man with a chainsaw who chases another man, so both represent atypical behaviour.

Moving on to the results from the caption generation sub-task, Figures \ref{vtt.bleu} and \ref{vtt.meteor} show the performance of runs submitted by 5 participating groups using the BLEU and METEOR metrics respectively.

The BLEU results in Figure~\ref{vtt.bleu} are difficult to interpret because, for example, multiple results from single sites are scattered throughout the results list whereas one would expect results from a single site to cluster as each site submits only minor variations of its own system for generating captions. This may be due to the issues associated with using BLEU for this tak, as mentioned earlier.  The METEOR results in Figure~\ref{vtt.meteor} show results for each site are indeed clustered and thus may be more reliable. However, for both BLEU and METEOR, trying to interpret the values of the system scores is impossible so their real value is in comparison only.

However, in order to give the reader some insight into the captions actually generated, Figure~\ref{vtt.sample.frame} shows a keyframe from one of the videos where a baby crawls forward across what appears to be a livingroom carpet, the camera zooms out to reveal a dog behind the baby and the dog does indeed mimic the way the baby crawls with its hind legs trailing behind it.  Below are the submitted captions for this video from across the groups (there are duplicate captions among the submissions). 

\begin{itemize}
\item a girl is playing with a baby
\item a little girl is playing with a dog
\item a man is playing with a woman in a room
\item a woman is playing with a baby
\item a man is playing a video game and singing
\item a man is talking to a car
\item A toddler and a dog
\end{itemize}

What this shows is that there are good systems that do well, and others that do not do well in terms of the captions that they generate, just as there are videos which are easier to caption than others, and each approach does well on some videos and badly on others, but not consistently so. For detailed information about the approaches and results, the reader should see the various site reports in the online workshop notebook \cite{tv16pubs}.

\subsection{Conclusions and Observations}

The first observation to make about the VTT pilot sub-tasks is that there was good participation from among TRECVid groups and that there are submitted captions and caption rankings from across the groups, which generate impressive results. Not all generated captions or caption rankings are correct or impressive, but there are enough good ones in the results of this pilot task to be encouraged. One of the quirks of the results was that B runs did better than A in matching and ranking while A did better than B in the semantic similarity, but that may be just an artefact of the annotation.

In terms of metrics used, METEOR scores are higher than BLEU, and in retrospect we should have used the CIDEr metric (Consensus-based Image Description Evaluation) \cite{vedantam2015cider} and as can be seen in their TRECVid papers, some participants did include this metric in their write-ups anyway. The CIDEr metric has been reported to show high agreement with consensus as assessed by humans. Using sentence similarity, the notions of grammaticality, saliency, importance and accuracy (precision and recall) are inherently captured by the metric. We plan to use again the three MT metrics including CIDEr in future evaluations so that a comparison can be made to assess which one can be more reliable as a metric.

STS, the semantics-based metric which we also used as a metric has some issues based on our anecdotal of its coverage for the language. This makes us ask what makes more sense, MT or semantic similarity, and which metric measures real system performance in a realistic application. To illustrate this, Figure~\ref{vtt.sts} shows the values of the STS metric where captions A and B are measured against each other, for each of the 2\,000 videos. One would expect that the A and B captions would be semantically similar, perhaps even identical and so we would hope for a large number of the 2\,000 similarity measures to be at, or close to, a value of 1,0.  Instead, as Figure~\ref{vtt.sts} illustates, the median similarity is only 0.545 with a disappointing tailoff of similarities close to a value of 0. That tells us that either the A and B annotators got things terribly wrong, which is unlikely given the quality assurance we used in producing the manual annotations, or the STS measure is having difficulty measuring similarity across just a short video caption, or the vocabulary used in the captioning creates difficulties for the STS computation.  Whatever the reason, STS similarity values would not add much value to interpreting the real performance of submitted runs.

One thing that became apparent as we looked at the approaches taken by different participants is that there are lots of available training sets for this task, including MSR-VTT, MS-COCO, Place2, ImageNet, YouTube2Text, and MS-VD. Some of these even have manual ground truth captions generated with Mechanical Turk such as the MSR-VTT-10k dataset \cite{xu2016msr} which has 10\,000 videos, is 41.2 h in duration  and has 20 annotations for each video.

This provides a rich landscape for those wishing to use machine learning in all its various forms within the VTT task and particpants in VTT have used all of these at some point.

Finally, while this was a pilot task in TRECVid in 2016, there are other video-to-caption challenges like the ACM MULTIMEDIA 2016 Grand Challenge where images from YFCC100M with captions were used in a caption-matching/prediction task for 36,884 test images. For participants in this Grand Challenge task, the majority of participants used CNNs and RNNs just as in VTT at TRECVid 2016, but unlike TRECVid, the ACM MM Grand Challenge setup does not give an opportunity for participants'
results to be aggregated and disseminated at the ACM MM Conference, so it is difficult  to gauge its overall impact in terms of comparison across participating systems, unlike in TRECvid where this happens at the workshop. We plan to continue working and improving the task next year with a similar setup and possible more human annotations.







